Optimizing Multi-DNN Inference on Mobile Devices through Heterogeneous Processor Co-Execution

Deep Neural Networks (DNNs) are increasingly deployed across diverse industries, driving demand for mobile device support. However, existing mobile inference frameworks often rely on a single processor per model, limiting hardware utilization and causing suboptimal performance and energy efficiency. Expanding DNN accessibility on mobile platforms requires adaptive, resource-efficient solutions to meet rising computational needs without compromising functionality. Parallel inference of multiple DNNs on heterogeneous processors remains challenging. Some works partition DNN operations into subgraphs for parallel execution across processors, but these often create excessive subgraphs based only on hardware compatibility, increasing scheduling complexity and memory overhead. To address this, we propose an Advanced Multi-DNN Model Scheduling (ADMS) strategy for optimizing multi-DNN inference on mobile heterogeneous processors. ADMS constructs an optimal subgraph partitioning strategy offline, balancing hardware operation support and scheduling granularity, and uses a processor-state-aware algorithm to dynamically adjust workloads based on real-time conditions. This ensures efficient workload distribution and maximizes processor utilization. Experiments show ADMS reduces multi-DNN inference latency by 4.04 times compared to vanilla frameworks.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> embed/equations/bbpairs.tex <==
\begin{equation}
\mathcal{M}_{f} ={ (\mathcal{H}_1, \mathcal{T}_1), (\mathcal{H}_2, \mathcal{T}_2) \dots (\mathcal{H}_n, \mathcal{T}_n) } \label{eq:bbpairs}
\end{equation}

==> embed/equations/charbonnier.tex <==
\begin{equation}
\mathcal{L}_{rec} = \sqrt{\|\boldsymbol{\mathrm{x}} - rec(enc(\boldsymbol{\mathrm{x}}))\|^2 + \epsilon^2}
\end{equation}

==> embed/equations/markovrepr.tex <==
\begin{equation}
\label{eq:dnnmarkovchain} 
I(X ; Y) \geq I\left(R_1 ; Y\right) \geq \ldots \geq I\left(R_n ; Y\right) \geq I(\tilde{Y} ; Y)
\end{equation}


==> embed/equations/min_angle_satellites.tex <==
\begin{equation}
\beta^{*} = 2 \times (180^{\circ}-(\theta + 90^{\circ}) - \arcsin({\frac{R_{\text{earth}} \cdot \sin{(90^{\circ}+\theta)}}{R_{\text{orbit}} + R_{\text{earth}}}})
%2\pi \cdot(2 \cdot (\pi-(\theta + \frac{\pi}{2} ) - \arcsin({\frac{R_{\text{earth}} \cdot \sin{(90^{\circ}+\theta)}}{R_{\text{orbit}} + R_{\text{earth}}}}))^{-1}
\end{equation}


==> embed/equations/modelling_em_latent.tex <==
\begin{equation}
p_{\tilde{\boldsymbol{\mathrm{y}}} \mid \tilde{\boldsymbol{\mathrm{z}}}}\left(\tilde{\boldsymbol{\mathrm{y}}} \mid \tilde{\boldsymbol{\mathrm{z}}}, \phi_h\right)=\prod_i\left(\mathcal{N}\left(\mu, \tilde{\sigma}_i^2\right) * \mathcal{U}\left(-\frac{1}{2}, \frac{1}{2}\right)\right)\left(\tilde{y}_i\right) \label{eq:memlatent}
\end{equation}

==> embed/equations/mutual_inf.tex <==
\begin{equation}
I(X;Y)=\int_{}\int_{} p(x,y) \log \left(\frac{p(x,y)}{p(x) p(y)}\right) dxdy \enspace .
\label{eq:mutualinf}
\end{equation}

==> embed/equations/pixels_per_seconds.tex <==
%\begin{equation}
%\frac{\text { Batch Size } \times \text { %Image Height } \times \text { Image Width } %\times \text { Bands }}{\text { Seconds per %Batch }}    
%\end{equation}

\begin{equation}
\text{PP/s} = \frac{B \times H \times W \times C}{\text{Seconds per Batch}}
\end{equation}


==> embed/equations/rd_objective.tex <==
\begin{equation}
\underset{P_{Y|X}}{\mathrm{min}}\; I(X;Y)\; \text{s.t.}\; \mathcal{D}(X,Y) \leq D_c \enspace ,
\label{eq:rdbasics}
\end{equation}

==> embed/equations/sideinfo_with_kps.tex <==
\begin{align}
    \boldsymbol{\hat{y}} &= Q(g_a({\boldsymbol{x};\theta})) \\
    \boldsymbol{y}_{kp} &= f_{ds}(k(\boldsymbol{x}) \odot \boldsymbol{x};\omega_{kp}) \\
    \boldsymbol{y}_{ca} &= a_c(\boldsymbol{y}_{kp}, \omega_{ca}) \\
    \hat{\boldsymbol{z}} &= Q(h_a(f_{ca}(\boldsymbol{y}_{kp}, \omega_{ca}); \theta_h)) \\
    p_{\hat{\boldsymbol{y}} \mid \hat{\boldsymbol{z}}}(\hat{\boldsymbol{y}} \mid \hat{\boldsymbol{z}}) &\leftarrow h_s\left(\hat{\boldsymbol{z}} ; \phi_h\right) \\
    \tilde{\boldsymbol{h}} &= g_s(\hat{\boldsymbol{y}};\phi)
\end{align}


==> embed/equations/time_to_orbit.tex <==
\begin{equation}
T_{\text{orbit}} =2\pi \sqrt{\frac{(R_{\text{orbit}} + R_{\text{earth}})^{3}}{GM}}
\end{equation}

==> embed/equations/transfer_cost_reduced_per_seconds_log.tex <==
\begin{equation}
\text{TCR/s} = \underbrace{\frac{B \times H \times W \times C}{\text{Seconds per Batch}}}_{\text{PP/s}} \times 
%\left(
\frac{\operatorname{log}(\text{bpp}_{\text{raw}})}{ \operatorname{log}(\text{bpp}_{\text{enc}})}
%\right)
\label{eq:tcrs}  
\end{equation}


==> embed/equations/transfer_cost_reduced_per_seconds_sub.tex <==
\begin{equation}
%\text{TCR/s} = \underbrace{\frac{B \times H \times W}{\text{Seconds per Batch}}}_{\text{PP/s}} 
\text{TCR/s} = \underbrace{\frac{\text{Image Dimension}}{\text{Seconds per Batch}}}_{\text{PP/s}} 
\times (\text{bpp}_{\text{raw}} - \text{bpp}_{\text{codec}})\label{eq:tcrs}  
\end{equation}


==> embed/equations/var_img_comp_obj_nohyper.tex <==
\begin{equation}
\mathbb{E}_{\boldsymbol{x} \sim p_{\boldsymbol{x}}} D_{\mathrm{KL}}\left[q \| p_{\tilde{\boldsymbol{\mathrm{y}}} \mid \boldsymbol{x}}\right]=\mathbb{E}_{\boldsymbol{x} \sim p_{\boldsymbol{x}}} \mathbb{E}_{\tilde{\boldsymbol{\mathrm{y}}} \sim q}-\mathrm{log}\;p(x|\boldsymbol{\tilde{\mathrm{y}}}) -\mathrm{log}\; p(\boldsymbol{\tilde{\mathrm{y}}})]\label{eq:compobjnosideinfo} 
\end{equation}


==> embed/equations/var_img_comp_obj_whyper.tex <==
\begin{align}
\mathbb{E}_{\boldsymbol{\mathrm{x}} \sim p_{\boldsymbol{\mathrm{x}}}} D_{\mathrm{KL}}\left[q \| p_{\boldsymbol{\mathrm{\tilde{y}}}, \boldsymbol{\mathrm{\tilde{z}}} \mid \boldsymbol{\mathrm{x}}}\right] &= \mathbb{E}_{\boldsymbol{\mathrm{x}} \sim p_{\boldsymbol{\mathrm{x}}}} \mathbb{E}_{\boldsymbol{\mathrm{\tilde{y}}}, \boldsymbol{\mathrm{\tilde{z}}} \sim q}\left[\log q(\boldsymbol{\mathrm{\tilde{y}}}, \boldsymbol{\mathrm{\tilde{z}}} \mid \boldsymbol{\mathrm{x}}) \right. \nonumber \\
& \left. -\log p_{\boldsymbol{\mathrm{x}} \mid \boldsymbol{\mathrm{\tilde{y}}}}(\boldsymbol{\mathrm{x}} \mid \boldsymbol{\mathrm{\tilde{y}}}) -\log p_{\boldsymbol{\mathrm{\tilde{y}}} \mid \boldsymbol{\mathrm{\tilde{z}}}}(\boldsymbol{\mathrm{\tilde{y}}} \mid \boldsymbol{\mathrm{\tilde{z}}})\right. \nonumber \\
& \left. -\log p_{\boldsymbol{\mathrm{\tilde{z}}}}(\boldsymbol{\mathrm{\tilde{z}}})\right] \label{eq:compobjwithsideinfo}
\end{align}


==> embed/equations/volume_captures.tex <==
\begin{equation}
%V_{\text{capture}} = \overbrace{\frac{S_w \cdot S_h \cdot R_{orbit}^{2}}{S_{GSD} \cdot F^{2}}}^{\text{Total Pixels}} \cdot \underbrace{S_{\text{bands}} \cdot S_{radio}}_{\text{Bits per Pixel}}  
V_{\text{capture}} = \overbrace{\frac{R^{2}_{\text{orbit}} \cdot \operatorname{tan}^2(S_{\text{fov}})}{S_w \cdot S_h}}^{\text{Total Pixels}} \cdot \underbrace{S_{\text{bands}} \cdot S_{\text{radio}}}_{\text{Bits per Pixel}}
\end{equation}


==> embed/equations/volume_pass.tex <==
\begin{equation}
V_{\text{pass}}  = \sum_{s^{(i)} \in \mathcal{G}_{j}} T_{\text{Orbit}} \cdot S^{(i)}_{\text{rate}} \cdot V^{(i)}_{\text{capture}}
\end{equation}

==> embed/media/fig_arch_components_org.tex <==
\begin{figure}[htb]
    \centering
    \includegraphics[width=\columnwidth]{figures/arch-org-comp.pdf}
    \caption{Network Organization and Components}
    \label{fig:archorgcomp}
\end{figure}

==> embed/media/fig_backbones_detection.tex <==
\begin{figure}[htb]
    \centering
    \includegraphics[width=\columnwidth]{figures/backbone-detection-models.pdf}
    \caption{Detection Pipeline for Evaluation}
    \label{fig:backbonesdetect}
\end{figure}

==> embed/media/fig_fool_comp_arch.tex <==
\begin{figure}[htb]
    \centering
    \includegraphics[width=\columnwidth]{figures/fool-comp-architecture-vert.pdf}
    \caption{The FOOL's Compression Architecture}
    \label{fig:foolcomparch}
\end{figure}

==> embed/media/fig_fool_detection_pipeline.tex <==
\begin{figure}[htb]
    \centering
    \includegraphics[width=\columnwidth]{figures/fool-hlvl-split-pt2-v3.pdf}
    \caption{Detection Pipeline for Evaluation}
    \label{fig:detectionpipeline}
\end{figure}

==> embed/media/fig_fool_hlvl.tex <==
\begin{figure}[htb]
    \centering
    \includegraphics[width=\columnwidth]{figures/fool-hlvl.pdf}
    \caption{Prediction High Level Overview}
    \label{fig:foolhlvl}
\end{figure}

==> embed/media/fig_fool_request_flow.tex <==
\begin{figure}[htb]
    \centering
    \includegraphics[width=\columnwidth]{figures/fool-hlvl-split-pt1.pdf}
    \caption{High-Level Inference Request Flow}
    \label{fig:foolhlvl}
\end{figure}

==> embed/media/fig_framework.tex <==
% TODO: Remove from here
% !TeX root = main.tex

\begin{figure}[t]
	\centering
%	\begin{minipage}[b]{0.23\textwidth}
%		\includegraphics[width=1\textwidth]{figs/live-streaming-buffer}
%		\subcaption{Jitter buffer size}
%	\end{minipage}
%	~
	\begin{minipage}[b]{0.48\textwidth}
		\includegraphics[width=1\textwidth]{figures/ecosystem.pdf}
		%\subcaption{Network and transcoding}
	\end{minipage}
	
	\caption{The service framework of existing EO ecosystems.}
	
	\label{fig:ecosystem}
	\vspace{-15pt}
\end{figure}

==> embed/media/fig_hd.tex <==
\begin{figure}[htb]
    \centering
    \includegraphics[width=\columnwidth]{figures/head_distillation_smoll_colorbrewer.pdf}
    \caption{Head Distillation Distortion Loss}
    \label{fig:hd}
\end{figure}

==> embed/media/fig_leftoverdep_vs_keypoints-whmap.tex <==
\begin{figure}[htb]
    \centering
    \includegraphics[width=\columnwidth]{figures/aerials_kps_vs_leftover2row-withhmap.png}
    \caption{Leftover Spatial Dependencies (middle left), Keypoints (middle right), Entropy Heatmap (right)}
    \label{fig:leftovervskeypoints}
\end{figure}

==> embed/media/fig_leftoverdep_vs_keypoints.tex <==
\begin{figure}[htb]
    \centering
    \includegraphics[width=\columnwidth]{figures/aerials_kps_vs_leftover2row.png}
    \caption{Leftover Dependencies (middle), Keypoints (right)}
    \label{fig:leftovervskeypoints}
\end{figure}

==> embed/media/fig_mult_backbones_mult_tasks.tex <==
\begin{figure}[htb]
    \centering
    \includegraphics[width=\columnwidth]{figures/mult-backbones-mult-tasks.pdf}
    \caption{Multiple Backbones with Multiple Tasks}
    \label{fig:multbbmulttasks}
\end{figure}

==> embed/media/fig_qual_analysis.tex <==
\begin{figure*}[htb]
    \centering
    % ATTENTION: Textwidths downscales it a tiny bit (original resolution doesn't quite fit but it doesn't destroy any visual ques that show the distortions
    \includegraphics[width=\textwidth]{figures/qual_analysis_4x1.pdf}
 %   \includegraphics[]{figures/qual_analysis.pdf}
    \caption{Visual Comparison between FOOL Image Recovery and a State-of-the-Art LIC model}
    \label{fig:qual_analysis}
\end{figure*}

==> embed/media/fig_qual_analysis_pt2.tex <==
\begin{figure*}[htb]
    \centering
    % ATTENTION: Textwidths downscales it a tiny bit (original resolution doesn't quite fit but it doesn't destroy any visual ques that show the distortions
    \includegraphics[width=\textwidth]{figures/qual_analysis_pt2.pdf}
 %   \includegraphics[]{figures/qual_analysis.pdf}
    \caption{Showcasing Potential of Recovery from Compressed Features with Finetuning for Perceptual Quality using LPIPS}
    \label{fig:qual_analysis_pt2}
\end{figure*}

==> embed/media/fig_recon_motivational.tex <==
\begin{figure}[htb]
    \centering
    \includegraphics[width=\columnwidth]{figures/resnet18-waddap1-gray.pdf}
    \caption{Discarding Information in Discriminative Tasks}
    \label{fig:reconmotivational}
\end{figure}

==> embed/media/fig_seq_vs_par.tex <==
\begin{figure}[htb]
    \centering
    \includegraphics[width=\columnwidth]{figures/seq-vs-par-exec.pdf}
    \caption{Sequential and Parallelizable Execution of DNNs}
    \label{fig:seqvsparexec}
\end{figure}

==> embed/media/fig_tensor_reshaping.tex <==
\begin{figure}[htb]
    \centering
    \includegraphics[width=\columnwidth]{figures/reshaping-tensors.pdf}
    \caption{Reshaping and Permuting Image Tensors}
    \label{fig:tensorreshape}
\end{figure}

==> embed/media/plot_comp_feature_perf_machine.tex <==
\begin{figure}[htb]
    \centering
    \includegraphics[width=\columnwidth]{plots/feat_comp_machine_percept.pdf}
    \caption{Compression Performance Feature Codecs}
    \label{plot:compfeatrdtask}
\end{figure}

==> embed/media/plot_comp_image_perf_machine.tex <==
\begin{figure}[htb]
    \centering
    \includegraphics[width=\columnwidth]{plots/image_comp_machine_percept.pdf}
    \caption{Compression Performance Image Codecs}
    \label{plot:compimagerdtask}
\end{figure}

==> embed/media/plot_cpu_gpu_usage_no_conc.tex <==
\begin{figure}[htb]
    \centering
    \includegraphics[width=\columnwidth]{plots/cpu_gpu_no_conc-orin-only.pdf}
    \caption{CPU (red) and GPU (blue) Usage of Encoder Network}
    \label{plot:cpugpunoconc}
\end{figure}

==> embed/media/plot_cpu_gpu_usage_with_conc.tex <==
\begin{figure}[htb]
    \centering
    \includegraphics[width=\columnwidth]{plots/cpu_gpu_conc-orin-only.pdf}
    \caption{CPU (red) and GPU (blue) Usage of Concurrent Pipeline}
    \label{plot:cpugpuwithconc}
\end{figure}

==> embed/media/plot_energy_cost_processing.tex <==
\begin{figure}[htb]
    \centering
    \includegraphics[width=\columnwidth]{plots/costs-to-double.pdf}
    \caption{Energy Cost of Compression Pipelines}
    \label{plot:energyprocessing}
\end{figure}

==> embed/media/plot_energy_transmission_savings.tex <==
\begin{figure}[htb]
    \centering
    \includegraphics[width=\columnwidth]{plots/transmission-savings-to-dec.pdf}
    \caption{Potential Energy Savings from Transmission}
    \label{plot:transmissionsavings}
\end{figure}

==> embed/media/plot_noisy_vs_lossy.tex <==
\begin{figure}[htb]
    \centering
    \includegraphics[width=\columnwidth]{plots/noisy_vs_lossy.pdf}
    \caption{Comparing Effect of Codec and Additive Noise}
    \label{plot:lossyvsnoisynoft}
\end{figure}

==> embed/media/plot_throughput_main.tex <==
\begin{figure}[htb]
    \centering
    \includegraphics[width=\columnwidth]{plots/throughput-main.pdf}
    \caption{Processing Throughput by Model Size}
    \label{plot:throughputmain}
\end{figure}

==> embed/media/plot_throughput_pilot.tex <==
\begin{figure}[htb]
    \centering
    \includegraphics[width=\columnwidth]{plots/throughput-pilot.pdf}
    \caption{Contrasting Throughput Measures}
    \label{plot:throughputpilot}
\end{figure}

==> embed/media/plot_tiles_to_saturation.tex <==
\begin{figure}[htb]
    \centering
    \includegraphics[width=\columnwidth]{plots/downlinked-volume.pdf}
    \caption{Downlinkable Data Volumes by Link}
    \label{plot:tilestosaturation}
\end{figure}

==> embed/tables/ablation.tex <==
\begin{table}[htb]
\centering
\caption{Ablations Comparisons for Lossless Prediction}
\label{tab:ablation}
\begin{tabularx}{\columnwidth}{@{\extracolsep{\fill}} 
l@{}
>{\raggedleft\arraybackslash} p{0.245\linewidth}@{}
>{\raggedleft\arraybackslash} p{0.286\linewidth}@{}
>{\raggedleft\arraybackslash} p{0.22\linewidth} }
Model & DOTA-2 (bpp \textdownarrow \textdownarrow) & SpaceNet-3 (bpp \textdownarrow \textdownarrow) & xView (bpp \textdownarrow \textdownarrow) \\ \toprule
\rowcolor[HTML]{EFEFEF} 
FOOL-L                         & 0.1843 & 0.1760 & 0.1822 \\
FOOL-M                         & 0.2110 & 0.1993 & 0.2032 \\
\rowcolor[HTML]{EFEFEF} 
FOOL-S                         & 0.2389 & 0.223  & 0.2290 \\ \hline
BSVBI-L                        & 0.3622 & 0.3440 & 0.3452 \\
\rowcolor[HTML]{EFEFEF} 
BSVBI-M                        & 0.3775 & 0.3605 & 0.3699 \\
BSVBI-S                        & 0.3889 & 0.3852 & 0.3909 \\ \hline
\rowcolor[HTML]{EFEFEF} 
NITA-L                         & 0.2209 & 0.1993 & 0.2032 \\
NITA-M                         & 0.2287 & 0.2193 & 0.2205 \\
\rowcolor[HTML]{EFEFEF} 
NITA-S                         & 0.2433 & 0.2386 & 0.2407 \\ \hline
NKPC-L                         & 0.2839 & 0.2712 & 0.2768 \\
\rowcolor[HTML]{EFEFEF} 
NKPC-M                         & 0.2926 & 0.2855 & 0.2883 \\
NKPC-S                         & 0.3116 & 0.3029 & 0.3112 \\ \bottomrule
\end{tabularx}
\end{table}

==> embed/tables/backbone-overview.tex <==
\begin{table}[htb]
\centering
\caption{Client Detection Model Architectures and Tasks }
\label{tab:backboneperformance}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{cccc}
\hline
Model                      & Task                               & mAP@50                       & mAP@50:95                    \\ \hline
                           & DOTA-2                             & 53.1                         & 33.1                         \\
                           & \cellcolor[HTML]{EFEFEF}SpaceNet-3 & \cellcolor[HTML]{EFEFEF}37.5 & \cellcolor[HTML]{EFEFEF}20.5 \\
\multirow{-3}{*}{YOLOv8-M} & xView                              & 38.2                         & 20.8                         \\ \hline
                           & \cellcolor[HTML]{EFEFEF}DOTA-2     & \cellcolor[HTML]{EFEFEF}53.1 & \cellcolor[HTML]{EFEFEF}33.1 \\
                           & SpaceNet-3                         & 37.5                         & 20.5                         \\
\multirow{-3}{*}{YOLOv8-L} & \cellcolor[HTML]{EFEFEF}xView      & \cellcolor[HTML]{EFEFEF}38.2 & \cellcolor[HTML]{EFEFEF}20.8 \\ \hline
                           & DOTA-2                             & 53.1                         & 33.1                         \\
                           & \cellcolor[HTML]{EFEFEF}SpaceNet-3 & \cellcolor[HTML]{EFEFEF}37.5 & \cellcolor[HTML]{EFEFEF}20.5 \\
\multirow{-3}{*}{YOLOv5-M} & xView                              & 38.2                         & 20.8                         \\
                           & \cellcolor[HTML]{EFEFEF}DOTA-2     & \cellcolor[HTML]{EFEFEF}53.1 & \cellcolor[HTML]{EFEFEF}33.1 \\
                           & SpaceNet-3                         & 37.5                         & 20.5                         \\
\multirow{-3}{*}{YOLOv5-M} & \cellcolor[HTML]{EFEFEF}xView      & \cellcolor[HTML]{EFEFEF}38.2 & \cellcolor[HTML]{EFEFEF}20.8
\end{tabular}%
}
\end{table}

==> embed/tables/comp_throughput_no_concurrent.tex <==
\begin{table}[htb]
\caption{Throughput Comparison Between Feature Codecs}
\label{tab:sumcompthroughput}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{ccccccc}
\hline
Model &
  \begin{tabular}[c]{@{}c@{}}PP/s \\ (Orin Nano)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}PP/s\\ (NX)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}PP/s\\ (TX2)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}PC/s \\ (Orin Nano)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}PC/s\\ (NX)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}PC/s\\ (TX2)\end{tabular} \\ \hline
\rowcolor[HTML]{EFEFEF} 
FOOL-L     & TBD & TBD & TBD & TBD & TBD & TBD \\
FOOL-M     & TBD & TBD & TBD & TBD & TBD & TBD \\
\rowcolor[HTML]{EFEFEF} 
FOOL-S     & TBD & TBD & TBD & TBD & TBD & TBD \\ \hline
Ablation-L & TBD & TBD & TBD & TBD & TBD & TBD \\
\rowcolor[HTML]{EFEFEF} 
Ablation-M & TBD & TBD & TBD & TBD & TBD & TBD \\
Ablation-S & TBD & TBD & TBD & TBD & TBD & TBD \\ \hline
\rowcolor[HTML]{EFEFEF} 
BSVBI-L    & TBD & TBD & TBD & TBD & TBD & TBD \\
BSVBI-M    & TBD & TBD & TBD & TBD & TBD & TBD \\
\rowcolor[HTML]{EFEFEF} 
BSVBI-S    & TBD & TBD & TBD & TBD & TBD & TBD \\ \hline
\end{tabular}%
}
\end{table}

==> embed/tables/complete_pipeline_throughput.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table}[]
\centering
\caption{Throughput Evaluation of Complete Pipeline}
\label{tab:completepipeline}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{ccccc}
\hline
Model &
  Device &
  \begin{tabular}[c]{@{}c@{}}Input Size\\ (MB)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Sequential\\ (MB/s)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Concurrent\\ (MB/s)\end{tabular} \\ \hline
                             & \cellcolor[HTML]{EFEFEF}Orin Nano & \cellcolor[HTML]{EFEFEF}42 & \cellcolor[HTML]{EFEFEF}4.2 & \cellcolor[HTML]{EFEFEF}4.2 \\
                             & TX2                               & 42                         & 4.2                         & 4.2                         \\
\multirow{-3}{*}{FOOL-L}     & \cellcolor[HTML]{EFEFEF}NX        & \cellcolor[HTML]{EFEFEF}42 & \cellcolor[HTML]{EFEFEF}4.2 & \cellcolor[HTML]{EFEFEF}4.2 \\
                             & Orin Nano                         & 42                         & 4.2                         & 4.2                         \\
                             & \cellcolor[HTML]{EFEFEF}TX2       & \cellcolor[HTML]{EFEFEF}42 & \cellcolor[HTML]{EFEFEF}4.2 & \cellcolor[HTML]{EFEFEF}4.2 \\
\multirow{-3}{*}{FOOL-M}     & NX                                & 42                         & 4.2                         & 4.2                         \\
                             & \cellcolor[HTML]{EFEFEF}Orin Nano & \cellcolor[HTML]{EFEFEF}42 & \cellcolor[HTML]{EFEFEF}4.2 & \cellcolor[HTML]{EFEFEF}4.2 \\
                             & TX2                               & 42                         & 4.2                         & 4.2                         \\
\multirow{-3}{*}{FOOL-S}     & \cellcolor[HTML]{EFEFEF}NX        & \cellcolor[HTML]{EFEFEF}42 & \cellcolor[HTML]{EFEFEF}4.2 & \cellcolor[HTML]{EFEFEF}4.2 \\ \hline
                             & Orin Nano                         & 42                         & 4.2                         & 4.2                         \\
                             & \cellcolor[HTML]{EFEFEF}TX2       & \cellcolor[HTML]{EFEFEF}42 & \cellcolor[HTML]{EFEFEF}4.2 & \cellcolor[HTML]{EFEFEF}4.2 \\
\multirow{-3}{*}{Ablation-L} & NX                                & 42                         & 4.2                         & 4.2                         \\
                             & \cellcolor[HTML]{EFEFEF}Orin Nano & \cellcolor[HTML]{EFEFEF}42 & \cellcolor[HTML]{EFEFEF}4.2 & \cellcolor[HTML]{EFEFEF}4.2 \\
                             & TX2                               & 42                         & 4.2                         & 4.2                         \\
\multirow{-3}{*}{Ablation-M} &
  \cellcolor[HTML]{EFEFEF}NX &
  \cellcolor[HTML]{EFEFEF}42 &
  \cellcolor[HTML]{EFEFEF}4.2 &
  \cellcolor[HTML]{EFEFEF}4.2 \\
                             & Orin Nano                         & 42                         & 4.2                         & 4.2                         \\
                             & \cellcolor[HTML]{EFEFEF}TX2       & \cellcolor[HTML]{EFEFEF}42 & \cellcolor[HTML]{EFEFEF}4.2 & \cellcolor[HTML]{EFEFEF}4.2 \\
\multirow{-3}{*}{Ablation-S} & NX                                & 42                         & 4.2                         & 4.2                         \\ \hline
                             & \cellcolor[HTML]{EFEFEF}Orin Nano & \cellcolor[HTML]{EFEFEF}42 & \cellcolor[HTML]{EFEFEF}4.2 & \cellcolor[HTML]{EFEFEF}4.2 \\
                             & TX2                               & 42                         & 4.2                         & 4.2                         \\
\multirow{-3}{*}{BSVBI-L}    & \cellcolor[HTML]{EFEFEF}NX        & \cellcolor[HTML]{EFEFEF}42 & \cellcolor[HTML]{EFEFEF}4.2 & \cellcolor[HTML]{EFEFEF}4.2 \\
                             & Orin Nano                         & 42                         & 4.2                         & 4.2                         \\
                             & \cellcolor[HTML]{EFEFEF}TX2       & \cellcolor[HTML]{EFEFEF}42 & \cellcolor[HTML]{EFEFEF}4.2 & \cellcolor[HTML]{EFEFEF}4.2 \\
\multirow{-3}{*}{BSVBI-M}    & NX                                & 42                         & 4.2                         & 4.2                         \\
                             & \cellcolor[HTML]{EFEFEF}Orin Nano & \cellcolor[HTML]{EFEFEF}42 & \cellcolor[HTML]{EFEFEF}4.2 & \cellcolor[HTML]{EFEFEF}4.2 \\
                             & TX2                               & 42                         & 4.2                         & 4.2                         \\
\multirow{-3}{*}{BSVBI-S}    & \cellcolor[HTML]{EFEFEF}NX        & \cellcolor[HTML]{EFEFEF}42 & \cellcolor[HTML]{EFEFEF}4.2 & \cellcolor[HTML]{EFEFEF}4.2 \\ \hline
\end{tabular}%
}
\end{table}

==> embed/tables/energy_consumption.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table}[htb]
\centering
\caption{Energy Usage and Savings from Rate Reduction}
\label{tab:energyconsumption}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{ccccc}
\hline
Device & Model & Inference (J) \textdownarrow \textdownarrow & Pipeline (J) \textdownarrow \textdownarrow & T. Red. (\%) \textuparrow \textuparrow \\ \hline
                            & \cellcolor[HTML]{EFEFEF}FOOL-S & \cellcolor[HTML]{EFEFEF}TBD & \cellcolor[HTML]{EFEFEF}TBD & \cellcolor[HTML]{EFEFEF}TBD \\
\multirow{-2}{*}{Orin Nano} & BSVBI-M                        & TBD                         & TBD                         & TBD                         \\ \hline
                            & \cellcolor[HTML]{EFEFEF}FOOL-S & \cellcolor[HTML]{EFEFEF}TBD & \cellcolor[HTML]{EFEFEF}TBD & \cellcolor[HTML]{EFEFEF}TBD \\
\multirow{-2}{*}{NX}        & BSVBI-M                        & TBD                         & TBD                         & TBD                         \\ \hline
                            & \cellcolor[HTML]{EFEFEF}FOOL-S & \cellcolor[HTML]{EFEFEF}TBD & \cellcolor[HTML]{EFEFEF}TBD & \cellcolor[HTML]{EFEFEF}TBD \\
\multirow{-2}{*}{TX2}       & BSVBI-M                        & TBD                         & TBD                         & TBD                         \\ \hline
\end{tabular}%
}
\end{table}

==> embed/tables/entropycoderperf.tex <==
\begin{table}[htb]
\centering
\caption{Performance for Entropy Coding Files}
\label{tab:entropycodingfiles}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{cccccccc}
\hline
Model &
  Device &
  Spatial Dim &
  \begin{tabular}[c]{@{}c@{}}Inference \\ (Files/s)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}File Size\\ (MB)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}rANS seq. \\ (MB/s)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}rANS w\textbackslash{}inf. \\ (MB/s)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}rANS w\textbackslash{}both. \\ (MB/s)\end{tabular} \\ \hline
 &
  \cellcolor[HTML]{EFEFEF}Orin Nano &
  \cellcolor[HTML]{EFEFEF}$500\times500$ &
  \cellcolor[HTML]{EFEFEF}4.20 &
  \cellcolor[HTML]{EFEFEF}0.420 &
  \cellcolor[HTML]{EFEFEF}420 &
  \cellcolor[HTML]{EFEFEF}420 &
  \cellcolor[HTML]{EFEFEF}420 \\
 &
  TX2 &
  $500\times500$ &
  4.20 &
  0.420 &
  420 &
  420 &
  420 \\
\multirow{-3}{*}{FOOL-L} &
  \cellcolor[HTML]{EFEFEF}NX &
  \cellcolor[HTML]{EFEFEF}$500\times500$ &
  \cellcolor[HTML]{EFEFEF}4.20 &
  \cellcolor[HTML]{EFEFEF}0.420 &
  \cellcolor[HTML]{EFEFEF}420 &
  \cellcolor[HTML]{EFEFEF}420 &
  \cellcolor[HTML]{EFEFEF}420 \\ \hline
 &
  Orin Nano &
  $500\times500$ &
  4.20 &
  0.420 &
  420 &
  420 &
  420 \\
 &
  \cellcolor[HTML]{EFEFEF}TX2 &
  \cellcolor[HTML]{EFEFEF}$500\times500$ &
  \cellcolor[HTML]{EFEFEF}4.20 &
  \cellcolor[HTML]{EFEFEF}0.420 &
  \cellcolor[HTML]{EFEFEF}420 &
  \cellcolor[HTML]{EFEFEF}420 &
  \cellcolor[HTML]{EFEFEF}420 \\
\multirow{-3}{*}{FOOL-M} &
  NX &
  $500\times500$ &
  4.20 &
  0.420 &
  420 &
  420 &
  420 \\ \hline
 &
  \cellcolor[HTML]{EFEFEF}Orin Nano &
  \cellcolor[HTML]{EFEFEF}$500\times500$ &
  \cellcolor[HTML]{EFEFEF}4.20 &
  \cellcolor[HTML]{EFEFEF}0.420 &
  \cellcolor[HTML]{EFEFEF}420 &
  \cellcolor[HTML]{EFEFEF}420 &
  \cellcolor[HTML]{EFEFEF}420 \\
 &
  TX2 &
  $500\times500$ &
  4.20 &
  0.420 &
  420 &
  420 &
  420 \\
\multirow{-3}{*}{FOOL-S} &
  \cellcolor[HTML]{EFEFEF}NX &
  \cellcolor[HTML]{EFEFEF}$500\times500$ &
  \cellcolor[HTML]{EFEFEF}4.20 &
  \cellcolor[HTML]{EFEFEF}0.420 &
  \cellcolor[HTML]{EFEFEF}420 &
  \cellcolor[HTML]{EFEFEF}420 &
  \cellcolor[HTML]{EFEFEF}420 \\ \hline
\end{tabular}%
}
\end{table}

==> embed/tables/entropycoderperfwbaselines.tex <==
\begin{table}[htb]
\centering
\caption{Concurrent Entropy Coding and Effect on TCR/s}
\label{tab:entropycodingfiles}
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{cccccc}
% \hline
\begin{tabularx}{\columnwidth}{@{\extracolsep{\fill}} 
% >{\raggedright\arraybackslash} p{0.14\linewidth}
l
>{\raggedleft\arraybackslash} p{0.14\linewidth}
r
>{\raggedleft\arraybackslash} p{0.118\linewidth}
>{\centering\arraybackslash} p{0.09\linewidth}
>{\raggedleft\arraybackslash} p{0.162\linewidth} }
Model & \makecell[c]{TCR/s\\$[$conc$]$} & \makecell[c]{TCR/s\\dec.} &
\makecell[c]{File Size\\(MB)}%\begin{tabular}[c]{@{}c@{}}File Size\\ (MB)\end{tabular} 
&  \makecell[c]{File/s} &
\makecell[c]{rANS conc.\\(MB/s)}%\begin{tabular}[c]{@{}c@{}}rANS conc.\\ (MB/s)\end{tabular} 
\\ 
\toprule %\hline
\rowcolor[HTML]{EFEFEF} 
FOOL-L  & $7.26 \cdot 10^{8}$ & \textbf{2.94\%} & 0.616 & 29 & 37.2                         \\
FOOL-M  & $7.57 \cdot 10^{8}$ & 1.28\%          & 0.462 & 31 & 38.3                         \\
\rowcolor[HTML]{EFEFEF} 
FOOL-S &
  \cellcolor[HTML]{EFEFEF}$1.32 \cdot 10^{9}$ &
  \cellcolor[HTML]{EFEFEF}1.06\% &
  0.383 &
  52 &
  38.8 \\ \hline
BSVBI-L & $5.96 \cdot 10^{8}$ & \textbf{2.88\%} & 0.822 & 37 & 37.6                         \\
\rowcolor[HTML]{EFEFEF} 
BSVBI-M & $7.15 \cdot 10^{8}$ & 1.37\%          & 0.617 & 42 & \cellcolor[HTML]{EFEFEF}39.6 \\
BSVBI-S & $6.91 \cdot 10^{8}$ & 1.28\%          & 0.437 & 58 & 40.1                         \\
\bottomrule %\hline
\end{tabularx}%
% }
\end{table}

==> embed/tables/hardware.tex <==
\begin{table}[htb]
\centering
\caption{Testbed Device Specifications}
\label{tab:hwconf}
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{ccc}
\begin{tabularx}{\columnwidth}{@{\extracolsep{\fill}} 
l %|
>{\raggedleft\arraybackslash} p{0.313\linewidth}
>{\raggedleft\arraybackslash} p{0.313\linewidth}
}
% \hline
\makecell[c]{Device}  & \makecell[c]{CPU} & \makecell[c]{GPU} \\ \toprule%\hline
\rowcolor[HTML]{EFEFEF} 
Ground Server    & 16x Ryzen @ 3.4 GHz & RTX 4090          \\
Edge (Nano Orin) & 6x Cortex @ 1.5 GHz & Amp. 512 CC 16 TC \\
% \multicolumn{1}{l}{Edge (Nano Orin)} & \multicolumn{1}{l}{6x Cortex @ 1.5 GHz} & \multicolumn{1}{l}{Amp. 512 CC 16 TC} \\
\rowcolor[HTML]{EDEDED} 
Edge (TX2)       & 4x Cortex @ 2 GHz   & Pas. 256 CC       \\
Edge (Xavier NX) & 4x Cortex @ 2 GHz   & Vol. 384 CC 48 TC \\ \bottomrule%\hline
% \end{tabular}%
\end{tabularx}
% }
\end{table}

==> embed/tables/impact_no_tiles.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table}[htb]
\centering
\caption{Effect of Number of TIles on Bpp}
\label{tab:impacttiles}
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{ccccc}
% \hline
\begin{tabularx}{\columnwidth}{@{\extracolsep{\fill}} 
% >{\raggedright\arraybackslash} p{0.14\linewidth} 
ccccc }
Model & Tiles & DOTA-2 (bpp \textdownarrow \textdownarrow) &
SpaceNet-3 (bpp \textdownarrow \textdownarrow) & xView (bpp \textdownarrow \textdownarrow) \\ \hline
& \cellcolor[HTML]{EFEFEF}3 & \cellcolor[HTML]{EFEFEF}0.2029 & \cellcolor[HTML]{EFEFEF}0.1931 & \cellcolor[HTML]{EFEFEF}0.1983 \\
& 4                         & 0.1918                         & 0.1863                         & 0.1886     \\
\multirow{-3}{*}{FOOL-L} &
  \cellcolor[HTML]{EFEFEF}5 &
  \cellcolor[HTML]{EFEFEF}\textbf{0.1843} &
  \cellcolor[HTML]{EFEFEF}\textbf{0.176} &
  \cellcolor[HTML]{EFEFEF}\textbf{0.1822} \\ \hline
                         & 3                         & 0.2205                         & 0.2188                         & 0.2203                         \\
                         & \cellcolor[HTML]{EFEFEF}4 & \cellcolor[HTML]{EFEFEF}0.2148 & \cellcolor[HTML]{EFEFEF}0.2079 & \cellcolor[HTML]{EFEFEF}0.2125 \\
\multirow{-3}{*}{FOOL-M} & 5                         & \textbf{0.2093}                & \textbf{0.201}                 & \textbf{0.2072}                \\ \hline
                         & \cellcolor[HTML]{EFEFEF}3 & \cellcolor[HTML]{EFEFEF}0.2501 & \cellcolor[HTML]{EFEFEF}0.420  & \cellcolor[HTML]{EFEFEF}0.420  \\
                         & 4                         & 0.2490                         & 0.420                          & 0.420                          \\
\multirow{-3}{*}{FOOL-S} &
  \cellcolor[HTML]{EFEFEF}5 &
  \cellcolor[HTML]{EFEFEF}\textbf{0.2468} &
  \cellcolor[HTML]{EFEFEF}\textbf{0.2385} &
  \cellcolor[HTML]{EFEFEF}\textbf{0.2447} \\ \hline
\end{tabularx}%
% }
\end{table}

==> embed/tables/missions.tex <==
\begin{table}[htb]
\centering
\caption{Constellation Link Conditions}
\label{tab:missions}
\begin{tabularx}{\columnwidth}{@{\extracolsep{\fill}} 
@{}l@{ }@{ }
l @{ }@{ }@{ }
l@{ }@{ }
>{\raggedleft\arraybackslash} p{0.11\linewidth}@{  }@{  }
>{\raggedleft\arraybackslash} p{0.07\linewidth}@{  }@{  }
>{\raggedleft\arraybackslash} p{0.138\linewidth} }
\makecell[l]{Oper.} & \makecell[l]{Constellation} & \makecell[l]{Link} & 
\makecell[r]{Rate\\(Mbps)} & \makecell[r]{Pass\\(s)} & \makecell[r]{Data Per\\Pass (GB)}
\\ \toprule
\rowcolor[HTML]{EFEFEF} 
Planet & Dove (3P/B13) & HSD 1         & 160  & 510 & 12.0  \\
Maxar  & WorldView     & WorldView-3   & 1200 & 600 & 90 \\
\rowcolor[HTML]{EFEFEF}
ESA    & Copernicus    & Sentinel 3A/B & 560  & 600 & 40.0  \\
% New row for NASA/USGS Landsat
\rowcolor[HTML]{FFFFFF}
NASA & Landsat & Landsat 8 & 440 & 120 & 39.6 \\
\hline
\end{tabularx}
\end{table}

==> embed/tables/n_codecs_params_macs.tex <==
% \def\myParColWidth{0.165}
\def\myParColWidth{0.165}
\begin{table}[ht]
\centering
\caption{Summary of Codec Parameter Distribution}
\label{tab:paramsmacsummary}
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{ccccc}
\begin{tabularx}{\columnwidth}{@{\extracolsep{\fill}} 
l %|
>{\raggedleft\arraybackslash}p{\myParColWidth\linewidth}
>{\raggedleft\arraybackslash}p{\myParColWidth\linewidth}
>{\raggedleft\arraybackslash}p{\myParColWidth\linewidth}
>{\raggedleft\arraybackslash}p{\myParColWidth\linewidth}}
% \toprule% \hline
Codec   & Pars. Total & Pars. Enc. & Pars. Dec. & Shared \\ 
% & \multicolumn{4}{c}{Parameter} \\ %\cline{2-5}
% Codec   & \makecell[r]{Total} & \thead[r]{Encoder} & \thead[r]{Decoder} & \thead[r]{Shared} \\ 
\toprule %\hline
FOOL-L  & 4.97M        & 1.19M       & 4.06M       & 0.28M         \\
\rowcolor[HTML]{EFEFEF} 
FOOL-M  & 4.33M        & 0.69M       & 3.83M       & 0.16M         \\
FOOL-S  & 3.91M        & 0.35M       & 3.66M       & 0.08M         \\
\rowcolor[HTML]{EFEFEF} 
SVBI-L  & 4.99M        & 1.25M       & 4.39M       & 0.65M         \\
SVBI-M  & 4.35M        & 0.72M       & 3.91M       & 0.29M         \\
\rowcolor[HTML]{EFEFEF} 
SVBI-S  & 3.95M        & 0.38M       & 3.71M       & 0.16M         \\
FP      & 7.03M        & 3.51M       & 3.51M       & 0.02M         \\
\rowcolor[HTML]{EFEFEF} 
%SHP     & 11.82M       & 8.31M       & 5.91M       & 2.41M         \\
MSHP    & 17.56M       & 14.06M      & 11.66M      & 8.15M         \\
JAHP    & 25.50M       & 21.99M      & 19.60M      & 16.10M        \\
\rowcolor[HTML]{EFEFEF} 
TinyLIC & 28.34M       & 21.23M      & 19.16M      & 12.05M        \\ 
\bottomrule%\hline
% \end{tabular}%
\end{tabularx}
% }
\end{table}

==> embed/tables/optim_config_memory.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table}[]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{ccccc}
\hline
Model                                                                                     & Device                            & Spatial Dims                    & Tiles                     & Memory (MB)                    \\ \hline
                                                                                          & \cellcolor[HTML]{EFEFEF}Orin Nano & \cellcolor[HTML]{EFEFEF}500x500 & \cellcolor[HTML]{EFEFEF}5 & \cellcolor[HTML]{EFEFEF}24,000 \\
                                                                                          & TX                                & 500x500                         & 5                         & 24,000                         \\
\multirow{-3}{*}{\begin{tabular}[c]{@{}c@{}}\{FOOL,\\ Ablation,\\ BSVBI\}-L\end{tabular}} & \cellcolor[HTML]{EFEFEF}NX2       & \cellcolor[HTML]{EFEFEF}500x500 & \cellcolor[HTML]{EFEFEF}5 & \cellcolor[HTML]{EFEFEF}24,000 \\ \hline
                                                                                          & Orin Nano                         & 500x500                         & 5                         & 24,000                         \\
                                                                                          & \cellcolor[HTML]{EFEFEF}TX        & \cellcolor[HTML]{EFEFEF}500x500 & \cellcolor[HTML]{EFEFEF}5 & \cellcolor[HTML]{EFEFEF}24,000 \\
\multirow{-3}{*}{\begin{tabular}[c]{@{}c@{}}\{FOOL,\\ Ablation,\\ BSVBI\}-M\end{tabular}} & NX2                               & 500x500                         & 5                         & 24,000                         \\ \hline
                                                                                          & \cellcolor[HTML]{EFEFEF}Orin Nano & \cellcolor[HTML]{EFEFEF}500x500 & \cellcolor[HTML]{EFEFEF}5 & \cellcolor[HTML]{EFEFEF}24,000 \\
                                                                                          & TX                                & 500x500                         & 5                         & 24,000                         \\
\multirow{-3}{*}{\begin{tabular}[c]{@{}c@{}}\{FOOL,\\ Ablation,\\ BSVBI\}-S\end{tabular}} & \cellcolor[HTML]{EFEFEF}NX2       & \cellcolor[HTML]{EFEFEF}500x500 & \cellcolor[HTML]{EFEFEF}5 & \cellcolor[HTML]{EFEFEF}24,000 \\ \hline
\end{tabular}%
}
\caption{Configurations That Maximize Throughput}
\label{tab:optimconfigmemory}
\end{table}

==> embed/tables/optim_config_memory_wthroughput.tex <==
\begin{table}[htb]
\centering
\caption{Throughput Comparison Between Feature Codecs}
\label{tab:optimconfigmemorywthroughput}
% \resizebox{\columnwidth}{!}{%% \begin{tabular}{ccccc}% \hline
\begin{tabularx}{\columnwidth}{@{\extracolsep{\fill}} 
c%@{ }@{ }
l >{\centering\arraybackslash}p{0.18\linewidth}@{ }@{ }
  >{\centering\arraybackslash}p{0.15\linewidth}@{ }@{ }%c
r }
Device &   Model &  Spatial Dim. & %Dimensions &
  Batch Size &  TCR/s \textuparrow\textuparrow \\ \toprule%\hline
 & FOOL-L & 600x600 & 4 & $7.4794\cdot10^{8}$ \\
 & \cellcolor[HTML]{EFEFEF}FOOL-M &
  \cellcolor[HTML]{EFEFEF}600x600 &
  \cellcolor[HTML]{EFEFEF}8 &
  \cellcolor[HTML]{EFEFEF}$7.6694\cdot10^{8}$ \\
\multirow{-3}{*}{Orin Nano} &
  \textbf{FOOL-S} &  600x600 &  8 &
  $\boldsymbol{1.3386\cdot10^{9}}$ \\ \hline
 & FOOL-L &  600x600 &  8 &  $7.5456\cdot10^{8}$ \\
 &\cellcolor[HTML]{EFEFEF}FOOL-M &
  \cellcolor[HTML]{EFEFEF}600x600 &
  \cellcolor[HTML]{EFEFEF}6 &
  \cellcolor[HTML]{EFEFEF}$8.1664\cdot10^{8}$ \\
\multirow{-3}{*}{NX} &  \textbf{FOOL-S} &  600x600 &  8 &
  $\boldsymbol{1.3422\cdot10^{9}}$ \\ \hline
 &\cellcolor[HTML]{EFEFEF}FOOL-L &
  \cellcolor[HTML]{EFEFEF}600x600 &
  \cellcolor[HTML]{EFEFEF}8 &
  \cellcolor[HTML]{EFEFEF}$2.3696\cdot10^{8}$ \\
 & FOOL-M &  600x600 &  8 &  $2.8067\cdot10^{8}$ \\
\multirow{-3}{*}{TX2} &
  \cellcolor[HTML]{EFEFEF}\textbf{FOOL-S} &
  \cellcolor[HTML]{EFEFEF}600x600 &
  \cellcolor[HTML]{EFEFEF}6 &
  \cellcolor[HTML]{EFEFEF}$\boldsymbol{4.0751\cdot10^{8}}$ \\ \hline
 &BSVBI-L &  600x600 &  8 &  $6.1419\cdot10^{8}$ \\
 &\cellcolor[HTML]{EFEFEF}\textbf{BSVBI-M} &
  \cellcolor[HTML]{EFEFEF}600x600 &
  \cellcolor[HTML]{EFEFEF}5 &
  \cellcolor[HTML]{EFEFEF}$7.2504\cdot10^{8}$ \\
\multirow{-3}{*}{Orin Nano} &
  BSVBI-S &  550x550 &  7 &  $6.9919\cdot10^{9}$ \\ \hline
 &\cellcolor[HTML]{EFEFEF}BSVBI-L &
  \cellcolor[HTML]{EFEFEF}600x600 &
  \cellcolor[HTML]{EFEFEF}8 &
  \cellcolor[HTML]{EFEFEF}$6.0007\cdot10^{8}$ \\
 &\textbf{BSVBI-M} &  600x600 &  6 &  $7.3717\cdot10^{8}$ \\
\multirow{-3}{*}{NX} &
  \cellcolor[HTML]{EFEFEF}BSVBI-S &
  \cellcolor[HTML]{EFEFEF}600x600 &
  \cellcolor[HTML]{EFEFEF}6 &
  \cellcolor[HTML]{EFEFEF}$7.0720\cdot10^{9}$ \\ \hline
 &BSVBI-L &  600x600 &  7 &  $1.7861\cdot10^{8}$ \\
 &\cellcolor[HTML]{EFEFEF}\textbf{BSVBI-M} &
  \cellcolor[HTML]{EFEFEF}600x600 &
  \cellcolor[HTML]{EFEFEF}6 &
  \cellcolor[HTML]{EFEFEF}$2.9978\cdot10^{8}$ \\
\multirow{-3}{*}{TX2} &  BSVBI-S &  600x600 &  7 &  $2.6818\cdot10^{8}$ \\ \bottomrule %\hline
\end{tabularx}%% }
\end{table}

==> embed/tables/recon_perf.tex <==
\begin{table}[htb]
\centering
\caption{Comparison Between Recovery and Image Codecs}
\label{tab:imagereconeval}
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{cccccc}
% \hline
\begin{tabularx}{\columnwidth}{@{\extracolsep{\fill}} 
% >{\raggedright\arraybackslash} p{0.14\linewidth}
l@{ }@{ }
>{\raggedleft\arraybackslash}p{0.125\linewidth}@{ }@{ }@{ }
>{\raggedleft\arraybackslash}p{0.17\linewidth}@{ }@{ }@{ }
>{\raggedleft\arraybackslash}p{0.12\linewidth}@{ }@{ }@{ }
>{\raggedleft\arraybackslash}p{0.1\linewidth}@{ }@{ }@{ }
>{\raggedleft\arraybackslash}p{0.18\linewidth} }
Model &
PSNR\textuparrow \textuparrow &
MS-SSIM\textuparrow\textuparrow &
LPIPS\textdownarrow\textdownarrow &
BPP\textdownarrow \textdownarrow &
Pred. Loss\textdownarrow\textdownarrow \\ \hline
FOOL       & 36.51                          & 15.43                         & 0.1480                          & 0.1808                         & \textbf{-}               \\
FOOL-FT &
  \cellcolor[HTML]{EFEFEF}35.56 &
  \cellcolor[HTML]{EFEFEF}14.57 &
  \cellcolor[HTML]{EFEFEF}0.1700 &
  \cellcolor[HTML]{EFEFEF}0.1808 &
  \cellcolor[HTML]{EFEFEF}\textbf{-} \\ \hline
FP-HQ      & 43.22                          & 25.07                         & 0.0896                         & 1.0470                          &  1.500                         \\
FP-MQ      & \cellcolor[HTML]{EFEFEF}35.56  & \cellcolor[HTML]{EFEFEF}16.55 & \cellcolor[HTML]{EFEFEF}0.2498 & \cellcolor[HTML]{EFEFEF}0.3200  & \cellcolor[HTML]{EFEFEF}7.508 \\ \hline
%SHP-HQ     & 43.77                          & 25.04                         & 0.0896                         & 1.0660                          &                          \\
%SHP-MQ     & \cellcolor[HTML]{EFEFEF}36.20 & \cellcolor[HTML]{EFEFEF}16.74 & \cellcolor[HTML]{EFEFEF}0.2395 & \cellcolor[HTML]{EFEFEF}0.2940  & \cellcolor[HTML]{EFEFEF} \\ \hline
MSHP-HQ    & 43.90                          & 25.20                         & 0.0841                         & 1.0370                          & 1.711                          \\
MSHP-MQ    & \cellcolor[HTML]{EFEFEF}36.45  & \cellcolor[HTML]{EFEFEF}16.83 & \cellcolor[HTML]{EFEFEF}0.2361 & \cellcolor[HTML]{EFEFEF}0.2787 & \cellcolor[HTML]{EFEFEF}7.180 \\ \hline
JAHP-HQ    & 43.95                          & 25.17                         & 0.0818                         & 1.0297                         &  1.504                        \\
JAHP-MQ    & \cellcolor[HTML]{EFEFEF}36.61  & \cellcolor[HTML]{EFEFEF}16.95 & \cellcolor[HTML]{EFEFEF}0.2303 & \cellcolor[HTML]{EFEFEF}0.2641 & \cellcolor[HTML]{EFEFEF}6.397 \\ \hline
TinyLIC-HQ & 44.52                          & 25.07                         & 0.0683                         & 1.0473                         &  1.602                        \\
TinyLIC-MQ &
  \cellcolor[HTML]{EFEFEF}37.42 &
  \cellcolor[HTML]{EFEFEF}17.27 &
  \cellcolor[HTML]{EFEFEF}0.2102 &
  \cellcolor[HTML]{EFEFEF}0.2899 &
  \cellcolor[HTML]{EFEFEF}5.499 \\ \hline
\end{tabularx}%
% }
\end{table}

==> sections/evaluation/compression.tex <==
\subsection{Rate Trade-off with Predictive Loss} \label{subsec:compperfmachine}
%We report predictive loss with mAP@50 since the absolute differences to lossless prediction are more apparent than mAP@[50:95] between the decreasing quality levels.
We report the predictive loss as a percentage point difference using mAP@50 on foundational detection models.
\subsubsection{Comparison to Image Codecs} \label{subsubsec:complic}
\Cref{plot:compimagerdtask} illustrates the trade-off between bpp (left is better) and predictive loss (top is better) for LIC models on each task separately.
\input{embed/media/plot_comp_image_perf_machine}
We primarily focus on how FOOL compares to existing SVBI to draw new insights from the novel additions and confirm that our results on aerial and satellite imagery datasets with one-stage detectors are consistent with previous findings on standardized terrestrial datasets~ \cite{frankensplit, es1, es2}. 
%The works in, already extensively demonstrate the advantage of SVBI over LIC models empirically when the objective is to minimize predictive loss for arbitrary tasks associated with a wide range of popular feature extractor architectures. 
 %
%Accordingly, we primarily focus on how FOOL compares to existing SVBI approaches to draw new insights.
%besides as a reference point to evaluate the image reconstruction quality (\Cref{subsubsec:evalreconfromlatent}), we focus 
%omit image codecs. Instead, we conduct more focused experiments on feature codecs to draw new insights. 
\subsubsection{Comparison to Feature Codecs} \label{subsubsec:compfeat}
\Cref{plot:compfeatrdtask} contrasts the trade-off between bpp and predictive loss for FOOL and BSVBI with progressively increasing sizes (i.e., capacity). 
%We set $T=5$ for FOOL, as it yields the best performance (\Cref{subsubsec:evalnumtiles}). 
%Interestingly, unlike for LIC models we observe comparable results for all three datasets.
The efficacy of compressing shallow features is best shown by comparing BSVBI and FOOL to MSHP, as they rely on the same entropy model. The highest quality MSHP model results in about 3-4\% predictive loss for DOTA-2. In contrast, the highest quality BSVBI-S model has 37x fewer encoder parameters but results in half the bitrate with no predictive loss.
\input{embed/media/plot_comp_feature_perf_machine}
Despite BSVBI demonstrating strong compression performance, FOOL significantly outperforms BSVBI across all configurations. FOOL-S has a ~51\% lower bitrate for configurations with lossless prediction than the comparatively large BSVBI-L. Relative to the FOOL model with matching capacity (FOOL-L), BSVBI-L has twice the bitrate.  
%We argue that this evidences that the novel components induce a correct bias, i.e., we scale the model's capacity beyond increasing model size. 
%TODO: Some comments about the different tasks and how the relationship may differ with LIC.
%Further, notice how the performance gap between FOOL and BSVBI increases as we increase capacity. FOOL can leverage the additional parameters more efficiently to find more powerful transforms. The primary difference between BSVBI and FOOL is that the former’s architecture increases depth with residual blocks. In contrast, FOOL’s architecture combines residual blocks with additional components. We argue that this evidences that the novel components induce a correct bias, i.e., we scale the model's capacity beyond increasing model size.
%Specifically, increasing the width of the layers that capture inter-tile dependencies and embed keypoints yields higher returns than exclusively expanding the width of residual blocks.
%\subsubsection{Number of Tiles} \label{subsubsec:evalnumtiles}
%FOOL considers inter-tile dependencies with weight sharing and lightweight convolutional attention (\Cref{subsubsec:tilecorrelations}). We briefly evaluate how the number of tiles influences rate performance by comparing lossless configurations and summarize the results in \Cref{tab:impacttiles}.
%\input{embed/tables/impact_no_tiles}
%As expected, the higher the model capacity, the better it can learn to leverage the inter-tile dependencies to lower bitrates. The rate reductions by increasing the tile count may seem marginal. However, even a slightly lower bpp results in considerable data volume reduction for large satellite images.
\subsubsection{Ablation Study} \label{subsubsec:ablation}
We may consider BSVBI an ablation, as FOOL extends BVSBI’s architecture by placing 3D attention layers between the residual blocks and a cross-attention layer to include context. The auxiliary networks $h_a$ and $h_s$ (\Cref{subsec:contextforfcomp}) are identical for FOOL and SVBI, i.e., three stacked residual blocks. Additionally, we perform ablation studies to assess by-component improvement and summarize the results for lossless predictions in \Cref{tab:ablation}.

\input{embed/tables/ablation}
The NITA models include the keypoint context without the inter-tile attention (ITA) layers. Analogous to BSVBI, we replace attention layers with residual blocks and match corresponding model sizes by increasing the depth and width of NITA models. 
%KPSI-Ablation and FOOL are (near) identical model architectures. The difference is whether we pass the weighted latent $\boldsymbol{\mathrm{y}}_{ca}$ to the quantizer or only use it to infer $\boldsymbol{\mathrm{z}}$. 
NKPC-Ablation drops components for embedding keypoints, i.e., it only includes the IT attention layers.
%Similar to \Cref{subsubsec:evalnumtiles}, we observe that larger models tend to benefit more from the attention layers. With lossless prediction, FOOL has a TODO\% lower bpp for the largest models, whereas it is only a TODO\% for the smallest models. 

The results show that relative to BSVBI, the task-agnostic context component contributes considerably more to rate reductions 
%(around 40\%) 
than the ITA layers
%(around 30\%) 
that leverage inter-tile spatial dependencies. 
%Moreover, KPSI shows that keypoints provide valuable context for side information (i.e., without further processing $\boldsymbol{\mathrm{y}}$) as it has up to TODO \% lower bpp than BSVBI for lossless configurations.
%Contrasting NKP-Ablation with IT-Ablation reveals that the keypoint context contributes considerably more to the overall improvement of FOOL over BSVBI. 
Still, we argue that the NTI-layers fulfill their purpose, to synergize with the partitioning strategy that maximizes processing throughput (\Cref{subsec:sysperf}).
\subsection{Image Reconstruction Quality} \label{subsec:compperfhuman}
We aim to demonstrate the feasibility of recovering presentable images from the compressed latent space of shallow features. We average results on DOTA-2, SpaceNet-3, and xView to reduce the bloat of reporting similar values summarize the results in \Cref{tab:imagereconeval}. For transparency, we exclusively select samples from the lower quartile across all measures to qualitatively showcase the reconstruction.
 
\input{embed/tables/recon_perf}
HQ refers to the weights with the highest available quality, and MQ refers to mid-quality weights that roughly match FOOL in PSNR. FOOL-FT finetunes the reconstruction model for an additional $2.5 \cdot 10^{5}$ iterations using LPIPS~\cite{lpips}. 
%
Unsurprisingly, the LIC models achieve significantly better scores across all reconstruction measures (i.e., PSNR, MS-SSIM, and LPIPS). The advantage of FOOL is that it has a considerably lower bitrate with no predictive loss on tasks for which it had no prior information.  Nonetheless, the results are considerably more interesting when contrasting FOOL to LIC models with mid-quality weights. Notice how FOOL matches reconstruction measures at no predictive loss and a 46-77\% \emph{lower} bitrate. Note that we did not find that the dataset significantly influences rate-distortion performance, except for a slight reduction in predictive loss (verified by training an FP model on the curation using the same setup as in \cite{begaint2020compressai}). Compression is a low-level vision task that generalizes well but may lack domain specificity when applying a standard rate-distortion reconstruction loss. In other words, the objective is the decisive difference between SVBI and LIC models. 
%
\input{embed/media/fig_qual_analysis}
To provide some intuition to the LPIPS measure, we select an image where FOOL-FT achieves considerably lower PSNR than TinyLIC and contrast the results in \Cref{fig:qual_analysis}.
Notice that the quality differences are most visible with fine-grained details, i.e., compared to TinyLic-HQ, TinyLic-MQ has a noticeable blur with some shadows completely missing in the bottom left. FOOL-FT preserves such details, despite lower PSNR, and this increase in perceptual quality is reflected in the LPIPS score.
\input{embed/media/fig_qual_analysis_pt2}
\Cref{fig:qual_analysis_pt2} further visualizes the potential of reliably recovering fine-grained from the compressed latent space.
Naturally, it should be possible to finetune the TinyLic-MQ to improve perceptual quality analogous to FOOl-FT. However, TinyLIC is still a significantly costlier model, with a worse rate and prediction performance. 
%
More pressingly, we stress that the \emph{reliability} of a restoration model is bound by the available signals in the compressed latent space. Accordingly, we deliberately avoid generative models that prioritize realism over structural integrity. 
%that may inflate the significance of our work with more visually pleasing images.
In particular, prioritizing realism over reliability defeats the primary purpose of image restoration, i.e., intervention by human experts in critical EO applications. A model outperforming experts does not imply that predictions may inexplicably be false. Specifically, where human cost is involved (e.g., disaster warning or relief~\cite{disasterwarning}) it is paramount that experts can trust the codec to not include extrapolated elements to an image.  
%For example, we can improve perceptual quality with GANs, 
%Naturally, it is possible to improve the quality targeting human perception for the LIC models by finetuning the decoder, but there are diminishing results as enough details of an object are already discernible (e.g., to verify unexpected predictions from detectors) for medium-quality models.
%The Entropic Student~\cite{es2} leverages the effectiveness of shallow features to train a feature compressor for (near-)arbitrary high-level vision tasks. FrankenSplit~\cite{frankensplit} takes this further to (near-)arbitrary target architectures and addresses the limitation of the HD distortion not resulting in a sufficient, but not minimal representation of $H$ with additional soft signals from deeper layers (i.e., saliency guidance). FOOL completes the previous observations by asserting that a sufficient reconstruction of shallow features resulting in comparable deep representations should imply a high perceptual similarity in the reconstructable input space~\cite{lpips}. 

We argue that our results adequately underpin the statements in \Cref{subsubsec:genshallowfeatures} and \Cref{subsubsec:machineandhumanperception}. In summary, if the salient regions align, compressing for model prediction requires more information than for human observation. Task specificity determines rate savings and not an entity's input interface. Targeting shallow features is minimally task-specific by relaxing the objective for lossless prediction on all possible tasks to those valuable for clients.

==> sections/evaluation/preamble.tex <==
\subsection{Experiment Design and Methodology} \label{sec:evalpreamble}
Our experiments reflect our aim to determine (i) the compression performance on aerial and satellite imagery without relying on prior knowledge and (ii) the feasibility of orbital inference.
\subsubsection{Testbed} \label{subsubsec:testbed} 
We benchmark~\cite{e2ebench} on an analytic and trace-driven~\cite{faassim} simulation based on results from a physical testbed with hardware summarized in \Cref{tab:hwconf}. 
The power consumption is capped at $15$W for the entire testbed.
\input{embed/tables/hardware}
%
Our simulation replicates a configurable CubeSat by imposing energy, memory, and bandwidth constraints. To simulate the downlink bottleneck with varying link conditions, parameterize link conditions and data volume (\Cref{subsec:oec}) using real-world missions~\cite{dovehsd, worldview3, sentinel3, landsat8specs} as summarized in \Cref{tab:missions}. %\Cref{tab:missions} summarizes the missions~\cite{dovehsd, worldview3, sentinel3, landsat8specs} and links we use experiment traces on. 
\input{embed/tables/missions}
 Due to the orthogonality of compression to systems-related challenges in OEC, we argue a focused simulation yields more insight results than running a full OEC simulator (e.g., \cite{denby2020}). 
%
% Research on system architectures for OEC is still an emerging field~\cite{oecsurvey2023,pfandzelter2021towards}. Further, different missions may run incomparable hardware configurations and scheduling strategies. For example, there is work on middleware for constellation coordination for task partitioning. In such systems, the resources for select satellites may be used exclusively for compression without preprocessing (e.g., cloud filtering)~\cite{kepler2020}.  
Our intention is for FOOL to facilitate OEC as an auxiliary method. Therefore, we demonstrate the bitrate reduction and resource usage trade-off for various configurations representing the heterogeneity of available compute resources and nanosatellite constellations. 
%
\subsubsection{Third-Party Detection Models} \label{subsubsec:detectors}
FOOL derives the basic approach to accommodate multiple backbones with a single encoder (\Cref{subsec:encmultisupport}) from FrankenSplit~\cite{frankensplit}. 
%
Foundational models (i.e., feature extractors or backbones) are interchangeable third-party components in SVBI. To complement previous work (\Cref{subsec:colinference}) and further show the flexibility of SVBI, we focus on modern YOLO variants~\cite{ultralytics}. 
%
\Cref{fig:backbonesdetect} illustrates the pipeline to represent third-party detectors we prepare before evaluating codecs. 

\input{embed/media/fig_backbones_detection}
While the work in \cite{frankensplit} did not explicitly evaluate object detection tasks, the support for two-stage detectors follows from the codec sufficiently approximating the representation of the feature extractor (i.e., the first stage). However, it is not apparent whether the general SVBI framework yields gains over image codecs when the targets are one-stage detectors. Therefore, to replicate a representative service for inference on aerial or satellite imagery, we apply simple transfer learning on open-source weights~\cite{ultralytics} for YOLOv5 and YOLOv8.
%


Image codecs pass a sample $dec(enc(\boldsymbol{\mathrm{x}})) = \boldsymbol{\hat{\mathrm{x}}}$ to the input layers of a target model. Feature codecs (i.e., SVBI methods) skip the shallow layers and pass $dec(enc(\boldsymbol{\mathrm{x}})) = \boldsymbol{\hat{\mathrm{h}}}$ to the deeper layers. Detection models with the same architecture share the frozen shallow layers (i.e., layers until the first non-residual connection). 

We select detection tasks to represent varying mission conditions.
DOTA-2~\cite{dota} for a more coarse-grained aerial task with comparatively lower Ground Sample Distance (GSD) and larger objects. SpaceNet-3~\cite{spacenet} for urban tasks (e.g., for traffic control) with high image resolutions. Lastly, xView~\cite{xview} for disaster response systems where detection models rely on fine-grained details. %\input{embed/tables/backbone-overview}
%\Cref{tab:backboneperformance} summarizes the detection model performance with the unprocessed test sets (i.e., without applying a codec). 
%The efficacy of SVBI methods is determined by how well they can find a minimal and sufficient representation for shallow features. 
%
To simplify the already intricate evaluation setup and to ease reproducibility, we deliberately refrain from more refined transfer learning methods. We merely require detection models with mAP scores that are moderately high to determine whether a codec can preserve fine-grained details for EO tasks on satellite imagery. For each architecture, we jointly finetune the deeper layers and train separate predictors that achieve around 35-65\% mAP@50. 
\subsubsection{Training \& Implementation Details} \label{subsubsec:impldetails}
To demonstrate that FOOL can handle detection tasks without relying on prior information (\Cref{subsec:limexistingcodecs}), we do not optimize the compression model with the training set of the prediction tasks (i.e., DOTA-2, SpaceNet-3, xView). Instead, 
we curate other aerial and satellite datasets~\cite{airbus, aerialcrowd, spacenet8, spacenet7, spacenet6, rareplanes, hrplanesv2, floodnet} that cover region and sensor diversity. SVBI does not rely on labels, i.e., replacing the curation with any diverse enough dataset from satellite imagery providers (e.g., Google Earth Engine) should be possible. 

We train one separate compression mode for each third-party detector using the shallow layers as teachers and verify whether the rate-distortion performance is comparable. Then, we freeze the encoder of the compression model for YOLOv5-L and discard all other encoders.
Lastly, we freeze the remaining encoder’s weights and (re-)train the separate decoders to demonstrate clients may request inference on variations (YOLOv5-M) or newer models as they emerge (YOLOv8).

We fix the tile resolution to $512 \times 512$ during training. We load samples as a video sequence for FOOL by grouping tiles from the same image in partitioning order with random transformations to fill any remaining spots. After training, the tensor shape (i.e., the number of tiles and the spatial dimensions) may vary for each separate sample. 
%Note that the NTC framework of LIC models generalizes exceptionally well since image compression is a low-level vision task that does not require capturing particular higher-level semantics. Hence, assuming comparable formats, the dataset domain (i.e., training with our curation) does not result in significantly better r-d performance. We verify the claim in \Cref{subsec:rdperformance}. While FOOL shares the same underlying principles as LIC, embedding keypoints as context and capturing inter-tile dependencies results in slight domain specificity (e.g., high-resolution samples we can partition to learn inter-tile dependencies).
%So even deeper configurations of FOOL’s convolutional layers cannot capture longer-ranging dependencies. This ensures a fair assessment of the performance gains from the novel additions, i.e., the lightweight local cross-attention and 3D-attention layers to embed inter-tile and keypoint content.  
%
We use PyTorch~\cite{pytorch}, CompressAI~\cite{begaint2020compressai}, and pre-trained detection models from Ultralytics~\cite{ultralytics}. To ensure reproducibility, we use torchdistill~\cite{matsubara2021torchdistill}. 
%Lastly, we extend an efficient implementation of rANS for entropy coding.
%
We use an Adam optimizer~\cite{kingma2014adam} with a batch size of $8$ and start with an initial learning rate of $1 \cdot 10^{-3}$, then gradually lower it to $1 \cdot 10^{-6}$ with an exponential scheduler. We first seek a weight for the rate term in \Cref{eq:compobjwithsideinfo} that results in lossless prediction with the lowest (best) bpp. Then, we progressively increase the term weight to evaluate trade-offs between rate and predictive loss. 
\subsubsection{Datasets Preparation} \label{subsubsec:datapreprocess}
The train sets for third-party detectors and the train sets for the compression models are strictly separated. However, we create square tiles for all datasets by partitioning the images with a configurable spatial dimension and applying 0-padding where necessary. 
%For example, a $980\times 980$ image would result in four $500 \times 500$ tiles.
%We do \textit{not} resize the tiles, i.e., smaller tile resolutions result in more samples. 
We extract bands from samples corresponding to RGB and convert them to 8-bit images, as to the best of our knowledge, there are no widespread open-source foundational models for detection with multispectral data yet. 
%
To ease direct comparisons, we convert the network detection labels of SpaceNet-3 by transforming the polygonal chains into bounding boxes. Lastly, since there are no publicly available labels for the xView and SpaceNet test sets, we create a 9:1 split on the train set. 
%Considering the complexity of processing a wide range of diverse datasets and formats, we provide the necessary scripts in the accompanying repository.
\subsubsection{Compression Performance Measures} \label{subsubsec:compmeasure}
To evaluate how codecs impact downstream task performance, we measure \emph{Predictive Loss} as the drop in mean Average Precision (mAP) by inputting decoded samples. We regard a configuration to result in \emph{lossless prediction} if there is less than 1\% difference in expected mAP@50. We confirm the observations from \cite{frankensplit} where the initial teacher only negligibly affects compression performance, and the predictive loss by a codec is comparable across target models (i.e., the retained information in shallow layers is similar across YOLO variations). Hence, for brevity, we aggregate the compression performance for each task separately, taking the highest predictive loss incurred on a detection model. 
%For example, if for xView, the predictive loss is 10\% for YOLOv5-M and 9\% for YOLOv8-L, we report it as 10\%. 
%and less than 0.1\% in mAP@[50:95]. 
%\input{embed/media/fig_backbones_detection}
%\Cref{fig:backbonesdetect} 
%illustrates the evaluation pipeline for predictive loss on detection models.
We train the image reconstruction model using the same configurations as \cite{swinir}, and compare it with LIC models using common measures (PSNR, MS-SSIM, LPIPS~\cite{lpips}).
%for the qualitative analysis.
\subsubsection{Baselines} \label{subsubsec:baselines}
We consider seminal work for image codecs as baselines with available open-source weights. Factorized Prior (FP)~\cite{fp} as a relatively small model without side information. (Mean-)scale hyperprior (SHP, MSHP)~\cite{shp, jahp} for drawing comparisons to side information in LIC, and Joint autoregressive and hierarchical priors (JAHP)~\cite{jahp} that further improves compression performance with an autoregressive context model. Lastly, TinyLIC~\cite{tinylic} represents recent work on efficient LIC design with state-of-the-art rate-distortion performance. 
\input{embed/tables/n_codecs_params_macs}
\Cref{tab:paramsmacsummary} summarizes parameter distributions between encoder and decoder components from LIC models. 
%TinyLIC is small relative to LIC models with comparable performance (e.g., \cite{chenlearnt} has over 90 million parameters). 

To draw comparisons to existing work on SVBI, we combine FrankenSplit~\cite{frankensplit} and the Entropic Student~\cite{es2} as a single baseline (BSVBI). We utilize FrankenSplit’s more efficient architecture design since it outperforms the latter without relying on finetuning the deeper layers. The encoder consists of stacked residual blocks (\Cref{subsec:modelbuildingblocks}), and the decoder is instantiated from a YOLOv5+ blueprint (C3 blocks~\cite{ultralytics}). We scale the capacity of BSVBI by including side information from LIC (MSHP) and increasing the width and depth to match the various FOOL configurations.
%FOOL extends BVSBI’s architecture by placing 3D attention layers between the residual blocks and a cross-attention layer to include context. 
%The auxiliary networks $h_a$ and $h_s$ (\Cref{subsec:contextforfcomp}) are identical for FOOL and SVBI, i.e., three stacked residual blocks. 
We train FOOL and BSVBI with the same dataset and training parameters (\Cref{subsubsec:impldetails}).
%Lastly, we fix $T=5$ for FOOL except in \Cref{subsubsec:evalnumtiles}, where we evaluate how the number of tiles impacts compression performance. 
%The S, M, and L widths (i.e., number of channels)  are 48, 42, and 36, respectively.

==> sections/evaluation/system.tex <==
\subsection{System Performance} \label{subsec:sysperf}
The following evaluates FOOL’s resource usage and how well it can address the downlink bottleneck. The methodology resembles how the system aids operators in determining the correct model size for a target device and estimating the increase in data volume relative to bent pipes. We do not apply vendor-specific optimization (e.g., TensorRT) to ensure transparent evaluation and keep the results reasonably platform agnostic. Instead, we instantiate all models dynamically with half-precision in the native PyTorch environment (\texttt{torch  1.14.0} with \texttt{CUDA 11.4.315}).
Image codecs are omitted for conciseness, as even the state-of-the-art for efficient LIC design still runs considerably slower than the largest SVBI models.
%requiring more memory despite showing lower rate reductions. 
%Moreover, we argue that the findings in \Cref{subsec:compperfmachine} sufficiently underpin the claims from \Cref{subsec:limexistingcodecs} that image codecs are inadequate for EO tasks. 
\subsubsection{Processing Throughput and Transfer Cost  Reduction} \label{subsubsec:evalinference}
We manually step through parts of the profiler (\Cref{subsec:resourcemaximation}) for evaluation and to show how it estimates gains in downlinkable data volume. 
%We can automate the profiling strategy from  but manually step through parts of the process for evaluation and 
%
Consider the results from measuring the friction between model sizes and input dimensions on processing throughput in \Cref{plot:throughputmain}. 
\input{embed/media/plot_throughput_main}
%
Notably, the processing throughput gain of FOOL-S over FOOL-M is significantly higher than FOOL-M over FOOL-L, despite FOOL-M having a comparable size difference to both models.   %Accordingly, the profiler should select a higher batch and tile size for FOOL-S than M or L. 

\input{embed/tables/optim_config_memory_wthroughput}
\Cref{tab:optimconfigmemorywthroughput} summarizes the configuration that maximizes 
profiler selection by TCR/s for all models on each device separately. Since bitrate variance is low between DOTA-2, SpaceNet-3, and xView, we average the bpp (\Cref{subsec:compperfmachine}) on the validation sets. The bold Model value indicates the adequate size of each model on a device, i.e., the model we will deploy to measure data volume downlinking in the following experiments. The bold TCR/s marks the highest overall value for a device, i.e., we can expect applying FOOL over BSVBI to result in considerably more downlinkable data on all devices. However, due to keypoint extraction and the ITA layers, FOOL's processing throughput is slower than BVSBI's. The overhead is particularly punishing for the most constrained device (i.e., the previous-generation TX2), where BSVBI-M has slightly higher TCR/s than FOOL-M, despite the latter's significantly better compression performance. Moreover, the profiler selects FOOL-S over FOOL-M/-L for the low-end current generation Orin Nano and high-end last-gen past generation NX. Conversely, the profiler decides on the mid-sized model for BSVBI across all devices despite FOOL's compression performance scaling better.
%, i.e., the overhead of scaling FOOL outweighs the lower bitrate.

Still, we argue that the results accentuate the findings from \Cref{subsubsec:compfeat}.
%and address the limitation discussed in \Cref{subsubsec:capacitycap}. 
Notice the contrast between TX2 and Nano Orin. One hardware generation was sufficient for the lowest-end device in the Jetson lineup to see a \emph{threefold} increase in TCR/s on FOOL-L over the last-generation midrange device. Thus, it is reasonable to claim that FOOL can (i) adequately leverage the current rapid progression of energy-efficient hardware improvement (i.e., with FOOL-M, L, and potentially larger variants)  and (ii) is flexible enough to be deployed on more constrained devices using the small FOOL-S that still achieve substantial rate reduction. 
% TODO: Maybe include a column with “Frame Size/s) to consider the frame deadline. 
\subsubsection{Model Inference with Concurrent Task Execution} \label{subsubsec:evalinferencewithconcurrent}
The following examines the claim in \Cref{sec:conctask}, i.e., whether FOOL’s compression pipeline can offset the runtime overhead of entropy coding. In other words, we evaluate whether interference between concurrent GPU and CPU-bound processes is negligible enough. We assume the worst case for interference, i.e., the CPU-bound processes constantly run concurrently by keeping them busy from an additional data stream when necessary. As all three devices have multicore CPUs and a dedicated GPU, we report results on the Nano Orin due to space constraints. 

\input{embed/tables/entropycoderperfwbaselines}
\Cref{tab:entropycodingfiles} summarizes the results from running the entire compression pipeline with concurrent task execution using the configurations that maximize TCR/s from \Cref{tab:optimconfigmemorywthroughput}. The bold values in the TCR/s dec. column indicates the size with the highest decrease.
A file includes all model artifacts output by the neural codec's DNN components for a single tile, i.e., the pipeline still needs to entropy code them to match the bpp in TCR/s calculations. 
%For example, if the batch size is 8, the pipeline entropy codes 8 separate files. 
%
File size refers to the storage requirements \emph{per tile} of the encoder output tensors, i.e., the data volume the rANS process encodes. 
We compute file size by a worst-case upper bound by the encoder output tensor dimensionality (\Cref{subsec:comparch}) without serialization formats that could exploit the sparsity of $\boldsymbol{\hat{\mathrm{y}}}$ and $\boldsymbol{\hat{\mathrm{z}}}$. 
There are two essential findings from the results. First, the rANS process can consume tasks considerably faster than the inference process can produce them, i.e., there is no risk of backpressure within the pipeline. Second, there is only a minimal percentage decrease in TCR/s across all devices and models relative to sequential execution. Hence, we argue that the pipeline successfully offsets the runtime overhead as claimed in \Cref{sec:conctask} even without relying on a precomputed lookup table (e.g., tANS in ZSTD~\cite{collet2018zstandard}).

The results are unsurprising when viewing the CPU (red) and GPU (blue) load of DNN inference without CPU-bound concurrent tasks in \Cref{plot:cpugpunoconc}. 
%
\input{embed/media/plot_cpu_gpu_usage_no_conc}
Since inference is GPU-bound, CPU usage is low even when the GPU is under maximal load. Contrast this with the CPU and GPU usage in \Cref{plot:cpugpuwithconc} where we monitor~\cite{e2ebench} usage while running the entire pipeline with the two concurrent processes.
\input{embed/media/plot_cpu_gpu_usage_with_conc}
If the CPU-bound processing task were to interfere with the DNN execution, resource usage should reveal frequent drops in GPU load. Comparing FOOL-L to S and M reveals some dependency between DNN size and CPU usage. For FOOL-L, two discernible drops in GPU usage suggest some interference, which may explain the 2.9\% decrease in TCR/s for FOOL-L and BSVBI-L. In contrast, there is no noticeable pattern difference in GPU load between \Cref{plot:cpugpuwithconc} and \Cref{plot:cpugpunoconc} for S and M variants, explaining the negligible 1-1.5\% TCR/s drop.
\subsubsection{Downlinkable Data Volume} \label{subsubsec:tilestosaturate}
We now compare how methods can alleviate the downlink bottleneck using the traces from previous experiments.
%according to constraints that represent existing missions. Specifically, we use the expected file sizes of entropy-coded samples 
%and the traces from runs with the link conditions of Lemur's TBD, Dove~\cite{dovehsd}'s HSD, and TBD's TBD.
\Cref{plot:tilestosaturation} visualizes the transferable volume per 
downlink pass. 
%
\input{embed/media/plot_tiles_to_saturation}
Notice the logarithmic scale, i.e., FOOL improves downlinking using bent pipes by over two orders of magnitude without relying on prior information on the downstream tasks or crude filtering methods. For example, given Maxar's WorldView-3 conditions~\cite{worldview3}, it would be possible to downlink roughly 9TB of sensor data per pass, before reaching downlink saturation. As a comparison, the state-of-the-art filtering method in~\cite{kodan} reports a 3$\times$ improvement, based on a definition of value. 
%
Note that to provide a realistic presentation of the opportunities SVBI provides, we assume that a nanosatellite processes tiles until reaching a downlink segment. Moreover, we disregard the ``computational deadline'', i.e., it can process all the data before reaching a ground segment. This is reasonable since there should always be enough data to process. If not produced by a single onboard sensor, constellations may designate certain satellites as compression nodes using reliable, high-capacity local communication channels~\cite{kepler2020}. Further, from the throughput evaluation and the orbital period, it is inferrable that even the low-end current-generation Orin Nano would barely miss the computational deadline. We remind the reader that the presented throughput measures represent a worst-case lower bound, as no vendor-specific software or hardware optimization was applied. 
%Note that this assumes that methods meet the ``computational deadline'', Nonetheless, 
%the TX2 misses the ``computational deadline'', Note that this , i.e., processing all data before reaching a ground segment. Nonetheless, Yet, the 
%this is nearly   the reader t
%We make no hard assumptions regarding sensor properties that determine the data volume. 
\subsubsection{Energy Consumption and Savings} \label{subsubsec:energycompsavings} 
%\textbf{Attention/TODO: 1) Needs explanation how we measure energy 2) The savings might be off, they're so outlandish, but some sanity checks confirm its within the realm of plausibility. Will pass calculations and experiment deetails to some colleague}
%
The following investigates the energy usage of the selected model for each device. As the GPU and CPU usage patterns are highly similar,
%(i.e., maxing out GPU usage, with the same CPU-bound processes executing in the background),,
we measure by the time it takes until a method can \emph{double} the downlinkable data. For example, if only downlinking 40 GB is possible with the unprocessed data, then we measure energy cost until the encoded size corresponds to 80 GB of raw captures. \Cref{plot:energyprocessing} summarizes the results.
%
\input{embed/media/plot_energy_cost_processing}
As expected, processing on TX2 requires more energy than on NX and Orin Nano as it is slower. Somewhat interesting is that the NX consumes more energy than the Orin Nano. As they execute the same models with comparable processing throughput, the results suggest that the newer Jetson lineup is more energy-efficient. 
%
Lastly, we measure savings from reduced transmission time, arguably an often undervalued advantage of compression. Admittedly, satellites will downlink as bandwidth permits, i.e., the transmission energy cost does not depend on the codec performance when there is saturation. Nonetheless, to intuitively show the amount of energy large volumes might require, we contrast with bent pipes in \Cref{plot:transmissionsavings}. 
%
\input{embed/media/plot_energy_transmission_savings}
Given the link conditions, we measure the difference in energy cost between transmitting until saturation and transmitting the corresponding raw volume from \Cref{plot:tilestosaturation}.
%
%TODO: Emphasize that this is not a real measurement, but just scaling the average measurement of transmitting Data per pass size 
%Downlinking the same raw data volume possible with a single downlink pass by using FOOL, would require up to approximately 150 Wh of energy.
